Finite Observations, Infinite Behaviour: bicategorical semantics for stateful monoidal processes

Time-dependent processes are often described by machines with an internal state which is updated as time evolves. An external observer cannot see this state and learns about a process only through finite observations of its inputs and outputs, each of which imposes a constraint on the trajectories the process can exhibit. We introduce a semantic construction in which two stateful processes have the same behaviour when they have the same constraints, as determined by finite observations, independent of their internal state. The construction is defined over any preorder-enriched monoidal category with a compatible notion of discarding, which we call a discard bicategory, capturing partial, non-deterministic, probabilistic, and quantum processes. The resulting category of behaviours provides a functorial semantics for free feedback categories in the sense of Katis, Sabadini, and Walters. For non-deterministic systems, we prove a categorified compactness theorem: every compatible family of finite observations between compact Hausdorff spaces extends uniquely and functorially to an infinite closed relation. Restricted to affine relations over finite fields, the compactness theorem recovers Willems' notion of behaviour for linear time-invariant systems.

==> style/tikz/bubbles.tex <==
% Phase-bubble pointer styles (wphase/bphase + curved bubble tails).
% Extracted from DZX.tikzdefs.
%
% Design (translucent, no seams, no doubling):
%  * A phase BUBBLE and ITS tail are drawn as ONE fill path (the rounded
%    rectangle and the tail are two subpaths of a single \path).  Because it is
%    a single fill operation, the union is painted once at the bubble's opacity:
%    the tail and bubble share the SAME translucency and their intersection is
%    the MAX (not the sum) -- no gap and no extra opacity.
%  * Two SEPARATE bubbles are separate fill ops, so they still composite/darken.
%  * Therefore the phase NODE itself carries only the TEXT (no fill); the fill
%    is produced by the tail edge.  Stand-alone phases with no tail use the
%    *solo* styles (wphasesolo/bphasesolo), which fill themselves.
%  * No borders anywhere.

%Bubble configs


% --- Adaptive tail base ---------------------------------------------------
% The tail base sits on the bubble edge; its length scales with the bubble's
% own size, clamped to [min,max].  Because the base runs ALONG the edge:
%   up/down arrows  (phasetonorth / phasetosouth): base is horizontal -> node WIDTH
%   left/right arrows (phasetowest / phasetoeast): base is vertical   -> node HEIGHT
% The base sits on the FLAT part of the bubble edge, i.e. the straight segment
% between the two rounded corners. We therefore scale off (dimension - edge
% inset), so short/narrow bubbles (e.g. the GAA axiom phases \(a\), \(a+b\),
% which are not \phasemat) get a small base that stays flush instead of
% spilling onto the rounded corners.
\newcommand{\wbubbleTailEdgeInset}{8pt} % ~2x bubble-base corner radius
\newcommand{\wbubbleTailWidthFrac}{0.65} % N/S base = this * (node width  - edge inset)
\newcommand{\wbubbleTailMinWidth}{2pt}
\newcommand{\wbubbleTailMaxWidth}{13pt}  % cap on N/S base width
\newcommand{\wbubbleTailHeightFrac}{0.55}% W/E base = this * (node height - edge inset)
\newcommand{\wbubbleTailMinHeight}{2pt}
\newcommand{\wbubbleTailMaxHeight}{8pt}  % cap on W/E base height

\newcommand{\wbubbleShiftWest}{0pt} % sideways nudge of W/E tails (0 = base centred on the edge)
\newcommand{\wbubbleShiftEast}{\wbubbleShiftWest}
% Spider nodes use a fixed circle geometry but outer sep=-1.8mm makes their
% normal connection anchors unreliable for phase arrows. Record the visible
% radius on each spider node so thin and thick outlines can both be met exactly.
\newcommand{\wbubbleThinSpiderTipRadius}{2.35mm}
\newcommand{\wbubbleThickSpiderTipRadius}{2.7mm}
\newcommand{\wbubbleSpiderTipRadius}{\wbubbleThinSpiderTipRadius}
\newcommand{\registerwbubbletipradius}[1]{%
  \expandafter\xdef\csname wbubbletipradius:\tikzlastnode\endcsname{#1}%
}
\newcommand{\setwbubbletipradius}{%
  \ifcsname wbubbletipradius:\tikztotarget\endcsname
    \edef\wbubbleSpiderTipRadius{\csname wbubbletipradius:\tikztotarget\endcsname}%
  \else
    \edef\wbubbleSpiderTipRadius{\wbubbleThinSpiderTipRadius}%
  \fi
}
\tikzstyle{phase-thin-spider}=[append after command={\pgfextra{\registerwbubbletipradius{\wbubbleThinSpiderTipRadius}}}]
\tikzstyle{phase-thick-spider}=[append after command={\pgfextra{\registerwbubbletipradius{\wbubbleThickSpiderTipRadius}}}]
\newcommand{\wbubbleCtrl}{2pt} % side curvature
% Tail base meets the bubble edge exactly. Because bubble+tail are one fill, the
% shared edge is interior to the fill -> no anti-alias gap and no doubling.
\newcommand{\wbubbleOverlap}{0pt}
\newcommand{\wbubbleTipSpread}{12}
\newcommand{\wbubbleTipCtrl}{3pt}
% Base is a straight chord on the edge (no bow into the bubble).
\newcommand{\wbubbleBaseBow}{0pt}
\newcommand{\bubbleWhiteBaseBow}{0pt}
\newcommand{\bubbleBlackBaseBow}{0pt}
\tikzstyle{use-bow-white}=[/utils/exec=\def\wbubbleBaseBow{\bubbleWhiteBaseBow}]
\tikzstyle{use-bow-black}=[/utils/exec=\def\wbubbleBaseBow{\bubbleBlackBaseBow}]


% ========= textures, shadows & layering =========
% Bubble FILL (and the tail) live on labeltextlayer: above the wires/spiders,
% but BELOW the phase node's text (which is on frontlayer). Only the rounded
% bubble casts an unscaled translated shadow on phaseshadowlayer; the tail does
% not cast a shadow, so it retains exactly the bubble fill colour and opacity.
% These shifts are deliberately 3pt because every picture is globally scaled
% to 0.5, yielding a visible 1.5pt offset in the rendered document.
\newcommand{\phaseShadowXShift}{2pt}
\newcommand{\phaseShadowYShift}{-2pt}
\newcommand{\phaseShadowOpacity}{.20}
\colorlet{addspiderphaseshadowcolor}{black!70!addspiderphasefillcolor}
\colorlet{copyspiderphaseshadowcolor}{black!70!copyspiderphasefillcolor}
\newcommand{\phaseShadowColor}{black}
\tikzstyle{bubble-skin}=[on layer=frontlayer, overlay]
\tikzstyle{bubble-layer-node}=[node on layer=frontlayer]

% Phase NODES are TEXT ONLY (fill is produced by the tail's union path).
\tikzstyle{bubble-white-node}=[bubble-skin, bubble-layer-node, /utils/exec=\def\phaseShadowColor{addspiderphaseshadowcolor}, draw=none, text=addspiderphasetextcolor, text opacity=1]
\tikzstyle{bubble-black-node}=[bubble-skin, bubble-layer-node, /utils/exec=\def\phaseShadowColor{copyspiderphaseshadowcolor}, draw=none, text=copyspiderphasetextcolor, text opacity=1]
% Stand-alone (tail-less) phases fill themselves, translucently.
\tikzstyle{bubble-white-node-solo}=[bubble-skin, bubble-layer-node, /utils/exec=\def\phaseShadowColor{addspiderphaseshadowcolor}, fill=addspiderphasefillcolor, draw=none, text=addspiderphasetextcolor, fill opacity=.85, text opacity=1]
\tikzstyle{bubble-black-node-solo}=[bubble-skin, bubble-layer-node, /utils/exec=\def\phaseShadowColor{copyspiderphaseshadowcolor}, fill=copyspiderphasefillcolor, draw=none, text=copyspiderphasetextcolor, fill opacity=.9, text opacity=1]
% Union (bubble+tail) fill: translucent, below the text.
\tikzstyle{bubble-white-path}=[on layer=labeltextlayer, overlay, fill=addspiderphasefillcolor, fill opacity=.85]
\tikzstyle{bubble-black-path}=[on layer=labeltextlayer, overlay, fill=copyspiderphasefillcolor, fill opacity=.9]
% ========= bubble base shape and phases =========
\newcommand{\bubbleCornerRadius}{4pt} % used both by the node and by the union path's rectangle
\newcommand{\bubbleMinimumDimension}{12pt} % 2*corner radius + tail minimum + 2pt clearance
\newcommand{\phasebubbleshadow}{%
  \begin{pgfonlayer}{phaseshadowlayer}%
    \path[
      overlay,
      draw=none,
      fill=\phaseShadowColor,
      fill opacity=\phaseShadowOpacity,
      rounded corners=\bubbleCornerRadius
    ]
      ($(\tikzlastnode.south west)+(\phaseShadowXShift,\phaseShadowYShift)$)
      rectangle
      ($(\tikzlastnode.north east)+(\phaseShadowXShift,\phaseShadowYShift)$);
  \end{pgfonlayer}%
}
\tikzstyle{bubble-base}=[
  rectangle, rounded corners=\bubbleCornerRadius, ultra thin,
  inner xsep=2pt, inner ysep=0.5pt, % smaller vertical padding
  minimum height=\bubbleMinimumDimension,
  minimum width=\bubbleMinimumDimension,
  font={\scriptsize\boldmath}, node on layer=frontlayer,
  append after command={\pgfextra{\phasebubbleshadow}}
]

% Phase bubbles connected by a tail (text only; fill comes from the tail).
\tikzstyle{wphase}=[bubble-base, bubble-white-node, tikzit category=ZX, tikzit fill=white, tikzit draw=white]
\tikzstyle{bphase}=[bubble-base, bubble-black-node, tikzit category=ZX, tikzit fill=black, tikzit draw=white]
% Stand-alone phase bubbles with NO tail (fill themselves).
\tikzstyle{wphasesolo}=[bubble-base, bubble-white-node-solo, tikzit category=ZX, tikzit fill=white, tikzit draw=white]
\tikzstyle{bphasesolo}=[bubble-base, bubble-black-node-solo, tikzit category=ZX, tikzit fill=black, tikzit draw=white]

% ========= pointer FILL alias (overridden by wrappers below) =========
\tikzstyle{bubble-tail}=[bubble-white-path] % default; wrappers override this

% \bubblerect: the bubble's own rounded rectangle as a fill subpath, so the
% tail's \path can fill (bubble UNION tail) in a single operation.
\newcommand{\bubblerect}{%
  [rounded corners=\bubbleCornerRadius]
  (\tikztostart.south west) rectangle (\tikztostart.north east)
  [sharp corners]%
}

% The bubble shadow is emitted when the phase node is placed. The attached
% arrow has no shadow; bubble and arrow are painted together exactly once.
\newcommand{\bubblefill}[1]{%
  \path[bubble-tail] \bubblerect #1;
}

% Compute the tail base length \WB from the live size of the phase node
% (\tikztostart) at draw time, clamped to [min,max].
\makeatletter
\newcommand{\setbubbletailwidth}{% \WB <- f(node WIDTH)   used by phasetonorth/south
  \pgfpointdiff{\pgfpointanchor{\tikztostart}{west}}{\pgfpointanchor{\tikztostart}{east}}%
  \edef\bubblenodedim{\the\pgf@x}%
  \pgfmathsetlengthmacro\WB{min(\wbubbleTailMaxWidth,%
        max(\wbubbleTailMinWidth,%
            \wbubbleTailWidthFrac*max(0pt, \bubblenodedim-\wbubbleTailEdgeInset)))}%
}
\newcommand{\setbubbletailheight}{% \WB <- f(node HEIGHT)  used by phasetowest/east
  \pgfpointdiff{\pgfpointanchor{\tikztostart}{south}}{\pgfpointanchor{\tikztostart}{north}}%
  \edef\bubblenodedim{\the\pgf@y}%
  \pgfmathsetlengthmacro\WB{min(\wbubbleTailMaxHeight,%
        max(\wbubbleTailMinHeight,%
            \wbubbleTailHeightFrac*max(0pt, \bubblenodedim-\wbubbleTailEdgeInset)))}%
}
\makeatother
% --------- BASE pointer geometry (no 'let' used) ---------


\tikzstyle{phasetosouth}=[
  draw=none,
  to path={
    \pgfextra{%
      \setbubbletailwidth
      \pgfmathanglebetweenpoints{\pgfpointanchor{\tikztotarget}{center}}{\pgfpointanchor{\tikztostart}{south}}%
      \edef\wbubang{\pgfmathresult}%
      \setwbubbletipradius
      \coordinate (wL)   at ($(\tikztostart.south)+(-.5*\WB, \wbubbleOverlap)$);
      \coordinate (wR)   at ($(\tikztostart.south)+(.5*\WB,  \wbubbleOverlap)$);
      \coordinate (wTip) at ($(\tikztotarget)+(\wbubang:\wbubbleSpiderTipRadius)$);
      \coordinate (cL) at ($ (wTip) + (\wbubang+\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \coordinate (cR) at ($ (wTip) + (\wbubang-\wbubbleTipSpread:\wbubbleTipCtrl) $);
      % bubble UNION tail, one fill -> one translucent shape (no seam/doubling)
      \bubblefill{
        (wL)
          .. controls ($(wL)+(\wbubbleCtrl,0)$) and (cL) .. (wTip)
          .. controls (cR) and ($(wR)+(-\wbubbleCtrl,0)$) .. (wR)
          .. controls ($(wR)+(0,\wbubbleBaseBow)$) and ($(wL)+(0,\wbubbleBaseBow)$) .. (wL)
        -- cycle
      }
    }%
    (\tikztostart) -- (\tikztotarget) \tikztonodes
  }
]

% ---------- NORTH ----------
\tikzstyle{phasetonorth}=[draw=none,
  to path={
    \pgfextra{%
      \setbubbletailwidth
      \pgfmathanglebetweenpoints{\pgfpointanchor{\tikztotarget}{center}}
                                 {\pgfpointanchor{\tikztostart}{north}}%
      \edef\wbubang{\pgfmathresult}%
      \setwbubbletipradius
      \coordinate (wL)   at ($(\tikztostart.north)+(-.5*\WB,-\wbubbleOverlap)$);
      \coordinate (wR)   at ($(\tikztostart.north)+(.5*\WB, -\wbubbleOverlap)$);
      \coordinate (wTip) at ($(\tikztotarget)+(\wbubang:\wbubbleSpiderTipRadius)$);
      \coordinate (cL) at ($ (wTip) + (\wbubang-\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \coordinate (cR) at ($ (wTip) + (\wbubang+\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \bubblefill{
        (wL)
          .. controls ($(wL)+(\wbubbleCtrl,0)$)      and (cL) .. (wTip)
          .. controls (cR) and ($(wR)+(-\wbubbleCtrl,0)$) .. (wR)
          .. controls ($(wR)+(0,-\wbubbleBaseBow)$)  and ($(wL)+(0,-\wbubbleBaseBow)$) .. (wL)
        -- cycle
      }
    }%
    (\tikztostart)--(\tikztotarget)\tikztonodes
  }
]

\tikzstyle{phasetowest}=[draw=none,
  to path={
    \pgfextra{%
      \setbubbletailheight
      \pgfmathanglebetweenpoints{\pgfpointanchor{\tikztotarget}{center}}
                                 {\pgfpointanchor{\tikztostart}{west}}%
      \edef\wbubang{\pgfmathresult}%
      \setwbubbletipradius
      \coordinate (wBase) at ($(\tikztostart.west)!\wbubbleOverlap!(\tikztostart.center)$);
      \coordinate (wT)    at ($(wBase)+(0,.5*\WB)$);
      \coordinate (wB)    at ($(wBase)+(0,-.5*\WB)$);
      \coordinate (wTip)  at ($(\tikztotarget)+(\wbubang:\wbubbleSpiderTipRadius)$);
      \coordinate (sT)    at ($(wT)+(\wbubbleShiftWest,0)$);
      \coordinate (sB)    at ($(wB)+(\wbubbleShiftWest,0)$);
      \coordinate (sTip)  at ($(wTip)+(\wbubbleShiftWest,0)$);
      \coordinate (sCT) at ($ (sTip) + (\wbubang+\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \coordinate (sCB) at ($ (sTip) + (\wbubang-\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \bubblefill{
        (sT)
          .. controls ($(sT)+(0,-\wbubbleCtrl)$) and (sCT) .. (sTip)
          .. controls (sCB) and ($(sB)+(0,\wbubbleCtrl)$) .. (sB)
          .. controls ($(sB)+(\wbubbleBaseBow,0)$) and ($(sT)+(\wbubbleBaseBow,0)$) .. (sT)
        -- cycle
      }
    }%
    (\tikztostart)--(\tikztotarget)\tikztonodes
  }
]

% ---------- EAST ----------
\tikzstyle{phasetoeast}=[draw=none,
  to path={
    \pgfextra{%
      \setbubbletailheight
      \pgfmathanglebetweenpoints{\pgfpointanchor{\tikztotarget}{center}}
                                 {\pgfpointanchor{\tikztostart}{east}}%
      \edef\wbubang{\pgfmathresult}%
      \setwbubbletipradius
      \coordinate (wBase) at ($(\tikztostart.east)!\wbubbleOverlap!(\tikztostart.center)$);
      \coordinate (wT)    at ($(wBase)+(0,.5*\WB)$);
      \coordinate (wB)    at ($(wBase)+(0,-.5*\WB)$);
      \coordinate (wTip)  at ($(\tikztotarget)+(\wbubang:\wbubbleSpiderTipRadius)$);
      \coordinate (sT)    at ($(wT)-(\wbubbleShiftWest,0)$);
      \coordinate (sB)    at ($(wB)-(\wbubbleShiftWest,0)$);
      \coordinate (sTip)  at ($(wTip)-(\wbubbleShiftWest,0)$);
      \coordinate (sCT) at ($ (sTip) + (\wbubang-\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \coordinate (sCB) at ($ (sTip) + (\wbubang+\wbubbleTipSpread:\wbubbleTipCtrl) $);
      \bubblefill{
        (sT)
          .. controls ($(sT)+(0,-\wbubbleCtrl)$) and (sCT) .. (sTip)
          .. controls (sCB) and ($(sB)+(0,\wbubbleCtrl)$) .. (sB)
          .. controls ($(sB)+(-\wbubbleBaseBow,0)$) and ($(sT)+(-\wbubbleBaseBow,0)$) .. (sT)
        -- cycle
      }
    }%
    (\tikztostart)--(\tikztotarget)\tikztonodes
  }
]


% family helpers
\tikzstyle{pointer-white}=[-, use-bow-white,
  bubble-tail/.style=bubble-white-path]

\tikzstyle{pointer-black}=[-, use-bow-black,
  bubble-tail/.style=bubble-black-path]


==> style/tikz/hbox.tex <==
% Directed Hadamard boxes (rhad/lhad/uhad/dhad and their thick g-variants).
% The palette styles live in DZX.tikzstyles; this file holds the machinery.
%
% Base `hadshape' is a plain (text-only) rectangle whose fill+border are drawn by
% a node `path picture' that rounds only the two HEAD-side corners
% (\hadcapnorth/south/east/west), leaving the other end flat and the two sides
% straight/orthogonal. Text is the node's own text, so it stays upright in every
% direction. Each corner-rounding path is a single closed \path whose corner
% rounding is toggled so exactly the two head corners are rounded.
\newcommand{\hadCapRadius}{4pt}
% The path picture is CLIPPED to the node's rectangle, so the stroke must sit
% strictly inside it (otherwise the border is clipped where the rounded arc nears
% the bbox edge). Inset every corner toward the centre by > half the line width.
\newcommand{\hadLineWidth}{.5pt}
\newcommand{\hadInset}{.4pt}
% Thick variant (grhad/glhad/gdhad/guhad): border matches the thick spiders
% (very thick = 1.2pt). Inset must exceed half this width so the stroke still
% fits inside the path-picture clip; outer sep is set to -\hadThickInset.
\newcommand{\hadThickLineWidth}{1.2pt}
\newcommand{\hadThickInset}{0.8pt}
% Extra padding on the HEAD axis (set by the directional styles as inner xsep for
% rhad/lhad or inner ysep for uhad/dhad), so the text is not crowded by the
% rounded cap. Only the head axis grows, keeping the box from getting much bigger.
\newcommand{\hadHeadPad}{3pt}
% Thick variant needs a bit more head padding: its wider border (and larger
% inset) consume more of the interior near the round cap.
\newcommand{\hadThickHeadPad}{4pt}
% Negative outer sep pulls wire connection points inward by the same inset, so
% wires meet the (inset) visible box edge instead of stopping at the bbox.
\tikzstyle{hadshape}=[shape=rectangle, draw=none, fill=none, text=hadamardtextcolor, minimum height=5pt, minimum width=5pt, inner sep=2pt, font={\scriptsize\boldmath}, anchor=center, outer sep=-\hadInset]
% corners (inset toward centre): start/route so only the HEAD corners round.
% SWi=(+,+) SEi=(-,+) NWi=(+,-) NEi=(-,-) offsets of \hadInset from the bbox corner.
\newcommand{\hadcapnorth}{\path[fill=hadamardfillcolor, draw=black, line width=\hadLineWidth, sharp corners, line join=round]
  let \p1=(path picture bounding box.south west), \p2=(path picture bounding box.north east) in
  ($(\x2,\y1)+(-\hadInset,\hadInset)$) -- ($(\x1,\y1)+(\hadInset,\hadInset)$) [rounded corners=\hadCapRadius] -- ($(\x1,\y2)+(\hadInset,-\hadInset)$) -- ($(\x2,\y2)+(-\hadInset,-\hadInset)$) [sharp corners] -- cycle;}
\newcommand{\hadcapsouth}{\path[fill=hadamardfillcolor, draw=black, line width=\hadLineWidth, sharp corners, line join=round]
  let \p1=(path picture bounding box.south west), \p2=(path picture bounding box.north east) in
  ($(\x1,\y2)+(\hadInset,-\hadInset)$) -- ($(\x2,\y2)+(-\hadInset,-\hadInset)$) [rounded corners=\hadCapRadius] -- ($(\x2,\y1)+(-\hadInset,\hadInset)$) -- ($(\x1,\y1)+(\hadInset,\hadInset)$) [sharp corners] -- cycle;}
\newcommand{\hadcapeast}{\path[fill=hadamardfillcolor, draw=black, line width=\hadLineWidth, sharp corners, line join=round]
  let \p1=(path picture bounding box.south west), \p2=(path picture bounding box.north east) in
  ($(\x1,\y1)+(\hadInset,\hadInset)$) -- ($(\x1,\y2)+(\hadInset,-\hadInset)$) [rounded corners=\hadCapRadius] -- ($(\x2,\y2)+(-\hadInset,-\hadInset)$) -- ($(\x2,\y1)+(-\hadInset,\hadInset)$) [sharp corners] -- cycle;}
\newcommand{\hadcapwest}{\path[fill=hadamardfillcolor, draw=black, line width=\hadLineWidth, sharp corners, line join=round]
  let \p1=(path picture bounding box.south west), \p2=(path picture bounding box.north east) in
  ($(\x2,\y1)+(-\hadInset,\hadInset)$) -- ($(\x2,\y2)+(-\hadInset,-\hadInset)$) [rounded corners=\hadCapRadius] -- ($(\x1,\y2)+(\hadInset,-\hadInset)$) -- ($(\x1,\y1)+(\hadInset,\hadInset)$) [sharp corners] -- cycle;}


==> style/tikz/multipliers.tex <==
% Signal-shaped multiplier "mat" plus the adaptive pointer-angle machinery that
% sizes the signal nodes. (Directed Hadamard boxes now live in hbox.tex.)
% Extracted from DZX.tikzdefs; depends on \arrowangle, \arrowscaling and the
% multiplierfillcolor definition in DZX.tikzdefs.

\tikzstyle{mat}=[shape=signal,  fill={multiplierfillcolor}, draw=black, minimum height=6pt, inner sep=1pt, font={\scriptsize\boldmath}, anchor=center, outer sep=-.1cm, signal pointer angle={\arrowangle}, scale={\arrowscaling}]
% Extra padding on the HEAD axis (set by lmat/rmat as inner xsep, umat/dmat as
% inner ysep) so the text is not crowded by the chevron point.
\newcommand{\matHeadPad}{2.5pt}

% Set \fastcompiletrue (after loading this file) to skip adaptive-angle
% computation and use \arrowangle everywhere. Speeds up large documents.
\newif\iffastcompile

% Adaptive pointer angle for signal nodes.
% Each style sets signal pointer angle to a string marker. A hook prepended to
% pgf@sh@s@signal detects the marker and computes a real angle from the live
% text-box dimensions before the signal geometry code reads the key.
%   adapt-vertical-angle   (dhad/uhad/dmat/umat): angle from text WIDTH
%   adapt-horizontal-angle (rhad/lhad/rmat/lmat): angle from text HEIGHT
% Formula: min(166, max(arrowangle, arrowangle + max(0, dim_pt - 5) * 1))
\makeatletter
\newdimen\@vertangledim
\def\pgf@sh@signal@adaptive@str{adaptive}
\def\pgf@sh@signal@adaptiveh@str{adaptive-h}
\def\pgf@sh@signal@setadaptiveangle{%
  \@vertangledim=\wd\pgfnodeparttextbox
  \edef\@vertangle@wpt{\strip@pt\@vertangledim}%
  \pgfmathparse{min(166.0, max(\arrowangle, \arrowangle + max(0.0, \@vertangle@wpt - 5.0) * 1))}%
  \pgfkeyssetvalue{/pgf/signal pointer angle}{\pgfmathresult}%
}%
\def\pgf@sh@signal@setadaptiveangleh{%
  \@vertangledim=\ht\pgfnodeparttextbox
  \advance\@vertangledim\dp\pgfnodeparttextbox
  \edef\@vertangle@wpt{\strip@pt\@vertangledim}%
  \pgfmathparse{min(166.0, max(\arrowangle, \arrowangle + max(0.0, \@vertangle@wpt - 5.0) * 1))}%
  \pgfkeyssetvalue{/pgf/signal pointer angle}{\pgfmathresult}%
}%
\global\let\pgf@sh@s@signal@orig=\pgf@sh@s@signal
\gdef\pgf@sh@s@signal{%
  \expandafter\ifx\csname pgfk@/pgf/signal pointer angle\endcsname\pgf@sh@signal@adaptive@str
    \iffastcompile
      \pgfkeyssetvalue{/pgf/signal pointer angle}{\arrowangle}%
    \else
      \pgf@sh@signal@setadaptiveangle
    \fi
  \else
    \expandafter\ifx\csname pgfk@/pgf/signal pointer angle\endcsname\pgf@sh@signal@adaptiveh@str
      \iffastcompile
        \pgfkeyssetvalue{/pgf/signal pointer angle}{\arrowangle}%
      \else
        \pgf@sh@signal@setadaptiveangleh
      \fi
    \fi
  \fi
  \pgf@sh@s@signal@orig
}%
\tikzset{adapt-vertical-angle/.style={signal pointer angle=adaptive}}
\tikzset{adapt-horizontal-angle/.style={signal pointer angle=adaptive-h}}
\makeatother


==> style/tikz/phasemat.tex <==
% Phase-label builder: \phasemat{<vector rows>}{<matrix rows>} typesets a
% vector-bar-matrix array sized to its contents. Pure math mode (no TikZ).
% Extracted from symbols.tex.
\ExplSyntaxOn
\seq_new:N \l__phasemat_vec_seq
\seq_new:N \l__phasemat_mat_seq
\seq_new:N \l__phasemat_col_seq
\tl_new:N  \l__phasemat_first_row_tl
\tl_new:N  \l__phasemat_colspec_tl
\int_new:N \l__phasemat_ncols_int

\NewDocumentCommand \phasemat { m m } {
  \ensuremath{ \__phasemat_build:nn {#1} {#2} }
}

\cs_new_protected:Nn \__phasemat_open_array:n { \begin{array}{#1} }
% Translucent separator rule. \pgfsetfillopacity only affects pgf fills, not a
% TeX \vrule, so we use the transparent package, which emits a real PDF
% transparency state that DOES apply to the rule. \begingroup..\endgroup keeps
% the transparency local to the rule.
\cs_new_protected:Nn \__phasemat_separator: {
  \begingroup
  \transparent{0.5}
  \vrule width \arrayrulewidth
  \endgroup
}

\cs_new_protected:Nn \__phasemat_build:nn {
  \seq_set_split:Nnn \l__phasemat_vec_seq { \\ } {#1}
  \seq_set_split:Nnn \l__phasemat_mat_seq { \\ } {#2}
  \tl_set:Nx \l__phasemat_first_row_tl
    { \seq_item:Nn \l__phasemat_mat_seq { 1 } }
  \seq_set_split:NnV \l__phasemat_col_seq { & } \l__phasemat_first_row_tl
  \int_set:Nn \l__phasemat_ncols_int { \seq_count:N \l__phasemat_col_seq }
  \int_compare:nNnTF { \seq_count:N \l__phasemat_vec_seq } = { 1 }
    {
      \int_compare:nNnTF { \l__phasemat_ncols_int } = { 1 }
        { \tl_set:Nn \l__phasemat_colspec_tl { @{}c@{\hspace{1.5pt}\__phasemat_separator:\hspace{1.5pt}}c@{} } }
        {
          \tl_set:Nn \l__phasemat_colspec_tl
            { @{\hspace{2pt}}c@{\hspace{\arraycolsep}\__phasemat_separator:\hspace{\arraycolsep}} }
          \int_step_inline:nn { \l__phasemat_ncols_int } {
            \tl_put_right:Nn \l__phasemat_colspec_tl { c }
          }
          \tl_put_right:Nn \l__phasemat_colspec_tl { @{\hspace{2pt}} }
        }
    }
    {
      \tl_set:Nn \l__phasemat_colspec_tl
        { @{\hspace{2pt}}c@{\hspace{\arraycolsep}\__phasemat_separator:\hspace{\arraycolsep}} }
      \int_step_inline:nn { \l__phasemat_ncols_int } {
        \tl_put_right:Nn \l__phasemat_colspec_tl { c }
      }
      \tl_put_right:Nn \l__phasemat_colspec_tl { @{\hspace{2pt}} }
    }
  \exp_args:NV \__phasemat_open_array:n \l__phasemat_colspec_tl
    \int_step_inline:nn { \seq_count:N \l__phasemat_vec_seq } {
      \seq_item:Nn \l__phasemat_vec_seq {##1}
      \char_generate:nn { 38 } { 4 }
      \seq_item:Nn \l__phasemat_mat_seq {##1}
      \int_compare:nNnF {##1} = { \seq_count:N \l__phasemat_vec_seq } { \\ }
    }
  \end{array}
}
\ExplSyntaxOff

